Weighted Alternating Tree Automata

We define weighted alternating tree automata â€” a generalization of weighted (non-alternating) tree automata, (unweighted) alternating tree automata, and weighted alternating (string) automata â€” over commutative semirings. We study their expressive power, and show that it is equivalent to that of weighted tree automata exactly when the employed semiring is locally finite. In our main result, we characterize the class of weighted tree languages defined by weighted alternating tree automata as the closure of the recognizable weighted tree languages under inverse tree homomorphisms.

==> eptcsdata.tex <==
\providecommand{\firstpage}{289}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.20}{10.4204/EPTCS.451.20}}
\pdfoutput=1

